Exotic Higgs Decay via AZ/HZ Channel: a Snowmass Whitepaper

While the conventional searches for the Higgs boson focus on its decays to Standard Model (SM) particles: gamma gamma, ZZ, WW, bb and tau tau, in this study, we explore the decays A --> HZ or H --> AZ. Such decays could appear in the exotic decay of the observed SM-like Higgs h --> AZ with a light A, or for extra Higgses in beyond the SM new physics scenarios with an extended Higgs sector. We study the exclusion bounds as well as discovery reach at the LHC for various combinations of (m_A, m_H) for the process: gg --> A/H --> HZ/AZ --> bbll for l =e, mu. We find that for 14 TeV LHC with 300 fb^{-1} integrated luminosity, the 95% C.L. limits on the cross-section for gg --> A/H --> HZ/AZ --> bbll vary between about 30 fb to a few fb for the parent heavy Higgs mass in the range 200 GeV to 600 GeV, while the limits for 5 sigma discovery are about 2-3 times larger. Comparing with the specific case of Next to Minimal Supersymmetric Standard Model, we find that this channel could be useful for heavy Higgs searches, especially for Higgs masses below 350 GeV.

==> references <==
1.  A --> hZ

%\cite{Lewis:2013fua}
\bibitem{Lewis:2013fua} 
  I.~M.~Lewis,
  %``Closing the Wedge with 300 fb^-1 and 3000 fb^-1 at the LHC: A Snowmass White Paper,''
  arXiv:1308.1742 [hep-ph].
  %%CITATION = ARXIV:1308.1742;%%

%\cite{Branco:2011iw}
\bibitem{Branco:2011iw} 
  G.~C.~Branco, P.~M.~Ferreira, L.~Lavoura, M.~N.~Rebelo, M.~Sher and J.~P.~Silva,
  %``Theory and phenomenology of two-Higgs-doublet models,''
  Phys.\ Rept.\  {\bf 516}, 1 (2012)
  [arXiv:1106.0034 [hep-ph]].
  %%CITATION = ARXIV:1106.0034;%%
  %185 citations counted in INSPIRE as of 21 Aug 2013

2. MSSM

%\cite{Nilles:1983ge}
\bibitem{Nilles:1983ge} 
  H.~P.~Nilles,
  %``Supersymmetry, Supergravity and Particle Physics,''
  Phys.\ Rept.\  {\bf 110}, 1 (1984).
  %%CITATION = PRPLC,110,1;%%
  %4165 citations counted in INSPIRE as of 21 Aug 2013

%\cite{Haber:1984rc}
\bibitem{Haber:1984rc} 
  H.~E.~Haber and G.~L.~Kane,
  %``The Search for Supersymmetry: Probing Physics Beyond the Standard Model,''
  Phys.\ Rept.\  {\bf 117}, 75 (1985).
  %%CITATION = PRPLC,117,75;%%
  %4033 citations counted in INSPIRE as of 21 Aug 2013

%\cite{Barbieri:1987xf}
\bibitem{Barbieri:1987xf} 
  R.~Barbieri,
  %``Looking Beyond the Standard Model: The Supersymmetric Option,''
  Riv.\ Nuovo Cim.\  {\bf 11N4}, 1 (1988).
  %%CITATION = RNCIB,11N4,1;%%
  %373 citations counted in INSPIRE as of 21 Aug 2013

3. 2HDM

%\cite{Branco:2011iw}
\bibitem{Branco:2011iw} 
  G.~C.~Branco, P.~M.~Ferreira, L.~Lavoura, M.~N.~Rebelo, M.~Sher and J.~P.~Silva,
  %``Theory and phenomenology of two-Higgs-doublet models,''
  Phys.\ Rept.\  {\bf 516}, 1 (2012)
  [arXiv:1106.0034 [hep-ph]].
  %%CITATION = ARXIV:1106.0034;%%
  %185 citations counted in INSPIRE as of 21 Aug 2013

\bibitem{type1}
H.E.~Haber, G.L.~Kane and T.~Sterling,
%``The Fermion Mass Scale And Possible Effects Of Higgs Bosons On Experimental
%Observables,''
Nucl.\ Phys.\ {\bf B161}, 493 (1979).
%%CITATION = NUPHA,B161,493;%%

  
 \bibitem{hallwise}
L.J.~Hall and M.B.~Wise,
Nucl.\ Phys.\ {\bf B187}, 397 (1981).
%%CITATION = NUPHA,B187,397;%%


\bibitem{type2}
J.F.~Donoghue and L.F.~Li,
%``Properties Of Charged Higgs Bosons,''
Phys.\ Rev.\ {\bf D19}, 945 (1979).
%%CITATION = PHRVA,D19,945;%%
  
4. NMSSM

%\cite{Ellis:1988er}
\bibitem{Ellis:1988er} 
  J.~R.~Ellis, J.~F.~Gunion, H.~E.~Haber, L.~Roszkowski and F.~Zwirner,
  %``Higgs Bosons in a Nonminimal Supersymmetric Model,''
  Phys.\ Rev.\ D {\bf 39}, 844 (1989).
  %%CITATION = PHRVA,D39,844;%%
  %655 citations counted in INSPIRE as of 21 Aug 2013

%\cite{Drees:1988fc}
\bibitem{Drees:1988fc} 
  M.~Drees,
  %``Supersymmetric Models with Extended Higgs Sector,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 4}, 3635 (1989).
  %%CITATION = IMPAE,A4,3635;%%
  %390 citations counted in INSPIRE as of 21 Aug 2013  

